Cyber Network Resilience against Self-Propagating Malware Attacks

Self-propagating malware (SPM) has led to huge financial losses, major data breaches, and widespread service disruptions in recent years. In this paper, we explore the problem of developing cyber resilient systems capable of mitigating the spread of SPM attacks. We begin with an in-depth study of a well-known self-propagating malware, WannaCry, and present a compartmental model called SIIDR that accurately captures the behavior observed in real-world attack traces. Next, we investigate ten cyber defense techniques, including existing edge and node hardening strategies, as well as newly developed methods based on reconfiguring network communication (NodeSplit) and isolating communities. We evaluate all defense strategies in detail using six real-world communication graphs collected from a large retail network and compare their performance across a wide range of attacks and network topologies. We show that several of these defenses are able to efficiently reduce the spread of SPM attacks modeled with SIIDR. For instance, given a strong attack that infects 97% of nodes when no defense is employed, strategically securing a small number of nodes (0.08%) reduces the infection footprint in one of the networks down to 1%.

==> auxinfo.tex <==

Printed plot: /home/simona/pwc/pwc-graph/src/defense/results_esorics/attack_plots_real/mitigate_3/port22/wc_8_20s_port22_comp3.png
            Degree    NB  NodeSplit+CI-Edge  CI-Edge  no defense
wc_1_500ms    0.02  0.08               0.13     0.31        0.97
wc_1_1s       0.01  0.07               0.13     0.30        0.97
wc_1_5s       0.01  0.04               0.12     0.29        0.92
wc_1_10s      0.02  0.08               0.14     0.30        0.99
wc_4_1s       0.02  0.08               0.14     0.31        0.96
wc_4_5s       0.02  0.08               0.14     0.30        0.97
wc_8_20s      0.02  0.08               0.13     0.30        0.97


Printed plot: /home/simona/pwc/pwc-graph/src/defense/results_esorics/attack_plots_real/mitigate_3/port80/wc_8_20s_port80_comp3.png
            Degree    NB  NodeSplit+CI-Edge  CI-Edge  no defense
wc_1_500ms    0.23  0.65               0.11     0.26        0.97
wc_1_1s       0.23  0.61               0.11     0.26        0.98
wc_1_5s       0.15  0.47               0.10     0.23        0.93
wc_1_10s      0.23  0.64               0.11     0.25        0.98
wc_4_1s       0.23  0.65               0.11     0.26        0.98
wc_4_5s       0.24  0.64               0.11     0.25        0.98
wc_8_20s      0.23  0.63               0.11     0.25        0.97

Printed plot: /home/simona/pwc/pwc-graph/src/defense/results_esorics/attack_plots_real/mitigate_3/port443/wc_8_20s_port443_comp3.png
            Degree    NB  NodeSplit+CI-Edge  CI-Edge  no defense
wc_1_500ms    0.10  0.25               0.14     0.40        0.99
wc_1_1s       0.11  0.26               0.14     0.40        0.97
wc_1_5s       0.08  0.17               0.13     0.39        0.93
wc_1_10s      0.10  0.27               0.14     0.40        1.00
wc_4_1s       0.11  0.27               0.14     0.40        1.00
wc_4_5s       0.11  0.26               0.14     0.40        0.98
wc_8_20s      0.10  0.25               0.14     0.39        0.98


==> questions.tex <==

--> \footnote{Protein-protein interaction networks also have very low transitivity.}.
did not see this anywhere; transitivity appears high in the biological graphs from Albert:2002:rmp, newman2003structure


newman, assortative mixing, connection with node removal
A network is said to show assortative mixing if the nodes in the network that have many connections tend to be connected to other nodes with many connections. Here we measure mixing patterns in a variety of networks and find that social networks are mostly assortatively mixed, but that technological and biological networks tend to be disassortative. We propose a model of an assortatively mixed network, which we study both analytically and numerically. Within this model we find that networks percolate more easily if they are assortative and that they are also more robust to vertex removal.

% As a side effect, it balances the load over two nodes instead of one, reducing the demand on the network through more efficient access to resources.

% Through node splits and migrations, providers achieve higher network capacity in response to increased data usage and demand on the network~\cite{nodesplits2022}.

reference, node splitting in bayesian networks
https://arxiv.org/pdf/1206.5251.pdf



\begin{table*}[!htpb]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Variant} & \multicolumn{4}{c}{AIC}\\ \cline{2-5}
&SI &SIS &SIR &SIIDR \\
\hline
wc-1-500ms &300 &30 &30 &-300\\
\hline
\end{tabular}
\caption{Model fitting for each WannaCry variant: lowest AIC scores for each SPM model.}
\label{tab:aic_scores_1}
\end{table*}


Robustness link. As a robustness measure, a larger λ1
indicates a more robust graph to random failures and attack,
along with increased susceptibility to virus propagation [4],
[7], [30], [51], [70], [77]. This is because the backup paths
and redundancy in a network are the same mechanisms that
allow a virus to quickly propagate.











